Incomplete Nested Dissection

We present an asymptotically faster algorithm for solving linear systems in well-structured 3-dimensional truss stiffness matrices. These linear systems arise from linear elasticity problems, and can be viewed as extensions of graph Laplacians into higher dimensions. Faster solvers for the 2-D variants of such systems have been studied using generalizations of tools for solving graph Laplacians [Daitch-Spielman CSC'07, Shklarski-Toledo SIMAX'08]. Given a 3-dimensional truss over $n$ vertices which is formed from a union of $k$ convex structures (tetrahedral meshes) with bounded aspect ratios, whose individual tetrahedrons are also in some sense well-conditioned, our algorithm solves a linear system in the associated stiffness matrix up to accuracy $\epsilon$ in time $O(k^{1/3} n^{5/3} \log (1 / \epsilon))$. This asymptotically improves the running time $O(n^2)$ by Nested Dissection for all $k \ll n$. We also give a result that improves on Nested Dissection even when we allow any aspect ratio for each of the $k$ convex structures (but we still require well-conditioned individual tetrahedrons). In this regime, we improve on Nested Dissection for $k \ll n^{1/44}$. The key idea of our algorithm is to combine nested dissection and support theory. Both of these techniques for solving linear systems are well studied, but usually separately. Our algorithm decomposes a 3-dimensional truss into separate and balanced regions with small boundaries. We then bound the spectrum of each such region separately, and utilize such bounds to obtain improved algorithms by preconditioning with partial states of separator-based Gaussian elimination.

==> proofofmain.tex <==
\begin{proof}[Proof of Theorem~\ref{thm:main}]
We bound the running time of Algorithm~\ref{alg:TrussSolver} $\textsc{TrussSolver}$.
The proof is similar to the proof of Theorem~\ref{thm:mainSmallAR}, except that in applying preconditioned conjugate gradient to solving a linear system in the Schur complement, 
 we use the union of the original trusses with large aspect ratios and the hollowings of the trusses with small aspect ratios as a preconditioner.

By Lemma~\ref{lem:kChunkND}, 
a Cholesky factorization of the preconditioner can be computed in time $O(n^{15/8}k^{17/4})$.
In each PCG iteration, solving a linear system in the preconditioner runs in time $O(n^{31/24}k^{17/6})$.
Furthermore, Definition~\ref{def:hollow} gives a bound of $O(n)$ on the condition
number, and in turn a bound of $O(n^{1/2} \log(1 / \epsilon))$ on
the number of PCG iterations via Theorem~\ref{thm:pcg}.
\todo{this only adds to $43 / 24$, which is not $15/8$!??!}
Thus, the total running time of Algorithm~\ref{alg:TrussSolver} is $O(n^{15/8} k^{17/4} \log (1/\eps))$.
\end{proof}


